Federated Learning in Genetics: Extended Analysis of Accuracy, Performance and Privacy Trade-offs

Machine learning on large-scale genomic or transcriptomic data is important for many novel health applications. For example, precision medicine tailors medical treatments to patients on the basis of individual biomarkers, cellular and molecular states, etc. However, the data required is sensitive, voluminous, heterogeneous, and typically distributed across locations where dedicated machine learning hardware is not available. Due to privacy and regulatory reasons, it is also problematic to aggregate all data at a trusted third party. Federated learning is a promising solution to this dilemma, because it enables decentralized, collaborative machine learning without exchanging raw data. In this paper, we perform comparative experiments with the federated learning frameworks TensorFlow Federated and Flower. Our test case is the training of disease prognosis and cell type classification models. We train the models with distributed transcriptomic data, considering both data heterogeneity and architectural heterogeneity. We measure model quality, robustness against privacy-enhancing noise and computational performance. We evaluate the resource overhead of a federated system from both client and global perspectives and assess benefits and limitations. Each of the federated learning frameworks has different strengths. However, our experiments confirm that both frameworks can readily build models on transcriptomic data, without transferring personal raw data to a third party with abundant computational resources. This paper is the extended version of https://link.springer.com/chapter/10.1007/978-3-031-63772-8_26.

==> cover_letter.tex <==
% For setting signatures and addresses in the cover letter
\setlength{\parindent}{0pt}


% Cover letter content
\begin{flushright}
    \textbf{Anika Hannemann} \\
    Center for Scalable Data Analytics and \\ Artificial Intelligence (ScaDS.AI) \\
    Dresden/Leipzig, Leipzig University, Germany \\
    hannemann@cs.uni-leipzig.de \\
\end{flushright}

\vspace{1cm}
    \today 
\vspace{1cm}

Valeria Krzhizhanovskaya \\
Editor-in-Chief \\
Journal of Computational Science \\

\vspace{0.5cm}

Dear Valeria Krzhizhanovskaya,

I am pleased to submit my manuscript titled "Federated Learning in Genetics: Extended Analysis of Accuracy, Performance and Privacy Trade-offs" for consideration in Journal of Computational Science. This paper presents the extended version of the paper \cite{hannemann2024federated} that was accepted for publication in ICCS 24. We extended the related work section and the experimental section. Figure \ref{fig:imbalanced_DL}, \ref{fig:AUC}, \ref{fig:time2} and Figure \ref{fig:memory2} are updated along with their description and analysis. 

We confirm that this manuscript has not been published elsewhere (except for its short version at ICCS 2024 conference proceedings) and is not under consideration by any other publication. We have no conflicts of interest to disclose.

Thank you for considering our submission. We look forward to your feedback and hope for a favorable response.

\vspace{0.5cm}

Sincerely, \\
Anika Hannemann \\
ScaDS.AI Dresden/Leipzig \\
\vspace{1cm}

\newpage % Start a new page for the main paper content
